AIR: Adaptive Interleaved Reasoning with Code in MLLMs

Following the paradigm shift initiated by OpenAI o3, interleaved reasoning with code to enhance multimodal large language models (MLLMs) has become a pivotal research frontier. The existing literature focuses primarily on tool-use within vision-perception tasks. However, such approaches typically rely on predefined heuristics for visual manipulation and are inherently incapable of addressing numerical computation problems due to their exclusive focus on visual operations. This paper empowers MLLMs with adaptive interleaved reasoning capabilities through extended reinforcement learning training on code-augmented complex numerical computation tasks. To this end, we propose a comprehensive three-component solution consisting of: a two-stage cold-start data construction pipeline, data filtering strategies for RL dataset curation, and an adaptive tool-invocation strategy leveraging a group-constrained reward function for interleaved reasoning trajectories. Extensive experiments demonstrate that after Reinforcement Learning training with the group-constrained reward function, performance improves by an average of 6.1 percentage points (pp) on evaluation benchmarks. Specifically, the accuracy for interleaved reasoning samples increases by 9.9 pp, and the overall success rate of tool-use exceeds 95%. Our data and code are available at: https://github.com/CongHan0808/AIR.git.

==> mm-retool/03-method-part4.tex <==


\subsection{Evaluation}
The evaluation of tool-calling proficiency constitutes a critical component of our study. 
We posit that tool-augmented reasoning effectively facilitates the inference process, and as such, it must maintain robust performance across established benchmarks. 
Given that adaptive tool-use is essential for maintaining stability during the training phase, we quantitatively assessed both the tool invocation rate and the success rate. 
To further validate model capabilities, we evaluated the quantitative metrics that reflect the capability improvement of interleaved reasoning compared with the baseline model.
% we utilized Claude to annotate the evaluation datasets, subsequently curating a specialized subset optimized for assessing tool-calling efficacy.

==> mm-retool/04_tab_res.tex <==
\begin{table*}[t]
\begin{center}
  \caption{Results on benchmarks. }  % 修正拼写错误
  \label{tab-main_result}
  \centering  % 替换center环境，实现无多余空白的居中
  \begin{small}
    \begin{tabular}{ccccccc}  % 8列表格，格式正确
      \toprule
      Model  & MathVista & MathVision & MathVerse & DynaMath & WeMath & LogicVista  \\
      \midrule
      Qwen2.5VL-7B &  64.1 & 24.6 & 40.9 & 53.5 & 30.7 & 44.3  \\  % 补充完整分隔符，换行符\\
      MM-Eureka &  72.6 & 28.1 & - &- & 21.8 & \\       % 新增换行符\\，补充完整分隔符
      VL-Rethinker &  \textbf{73.7} & 28.4& - &- & 36.3 & \\       % 新增换行符\\，补充完整分隔符
      Thyme &  70.0 & 27.6 & - &-  &39.3 & \\       % 新增换行符\\，补充完整分隔符
      DeepEyesV2 &  71.9 & \textbf{28.9} & \textbf{52.7} &57.2 & 38.1 & \\       % 新增换行符\\，补充完整分隔符
      \textbf{\ourmethod}-SFT &  67.8& 27.9 & 43.5& 48.3& \textbf{43.9} & 43.17 \\
      \textbf{\ourmethod} &  72.2& 28.4 &48.6 & \textbf{57.5} & 40.6 & \textbf{47.7} \\ 
      \bottomrule
    \end{tabular}
  \end{small}
  % 建议删除\vskip -0.1in，如需调整间距用规范参数设置
\end{center}
\end{table*}  % 修正环境结尾，与开头table*匹配\subsection{Main Results}


\begin{table*}[t]
\begin{center}
  \caption{Comparison Under the Interleaved Reasoning Scenario.} 
  % \caption{交错推理场景下模型性能比较。} 
  \label{tab-interreasoning_result}
  \centering  % 替换center环境，实现无多余空白的居中
  \begin{small}
    \begin{tabular}{ccccccccc}  % 8列表格，格式正确
      \toprule
      Model  & MathVista & MathVision & MathVerse & DynaMath & WeMath & LogicVista &Avg.I.R. & Avg. All \\
      \midrule
      % Qwen2.5VL-7B &63.6 &17.8 &35.2 &53.6 &70.8 &44.8 &49.4 & 47.6 \\
      \textbf{\ourmethod}-SFT &  63.6& 20.4 &42.6& 46.2& 74.6 & 51.7 &46.4 & 45.8 \\ %49.9
      \ourmethod &  67.5& 25.7 &56.5 & 60.0 & 72.3 & 44.8 &56.3 & 49.2 \\ %54.5
      \bottomrule
    \end{tabular}
  \end{small}
  % 建议删除\vskip -0.1in，如需调整间距用规范参数设置
\end{center}
\end{table*}  % 修正环境结尾，与开头table*匹配\subsection{Main Results}


\begin{table*}[t]
\begin{center}
  \caption{Comparison between interleaved reasoning ratio, code execution accuracy and Evaluation Set Metrics. 
    \textbf{Model-low/mid/high} denote the levels of interleaved reasoning ratio of the model. 
    For each specific dataset, the two numerical values respectively represent the proportion of interleaved reasoning data and the execution accuracy of tools.
    \textbf{Avg.Acc.} indicates the average accuracy of the corresponding model on all data within each dataset.

  }  % 修正拼写错误
  \label{tab-toolcall-ratio}
  \centering  % 替换center环境，实现无多余空白的居中
  \begin{small}
    \begin{tabular}{cccccccc}  % 8列表格，格式正确
      \toprule
      Model  & MathVista & MathVision & MathVerse & DynaMath & WeMath & LogicVista & Avg. Acc.  \\
      \midrule
      model-low & 8.6\% / 97.7\% & 4.1\% / 85.9\% & 7.5\% / 96.6\% & 12.5\% / 95.3\% & 3.7\% / 99.1\% & 3.4\%/93.3\% & 48.4 \\
      model-mid &15.4\% / 98.1\% & 7.8\% / 86.9\%  &13.7\%/98.2\% & 19.1\%/95.0\% & 7.5\% / 99.0\% & 6.5\% /100\% & 48.8 \\
      model-high &79.6\%/95.3\% & 56.7\%/91.9\% & 62.2\%/96.1\% & 76.7\% / 91.8\% & 70.0\%/98.2\% & 65.3\% / 92.4\% & 49.0 \\
      \bottomrule
    \end{tabular}
  \end{small}
\end{center}
  % 建议删除\vskip -0.1in，如需调整间距用规范参数设置
\end{table*}



\begin{table}[!htbp]      % 补全位置参数，解决表格乱跑/失踪
  \centering             % 置顶写，标题+表格一起居中，格式规范
  \small                 % 缩小字体，表格更紧凑，无结束命令！
  \caption{Ablation study for RL data.}
  \label{tab-ablation_data}
  % tabular列数修正：表头5列 → {lcccc} 刚好匹配，无多余列
  \begin{tabularx}{0.95\columnwidth}{c@{\hspace{0.5em}}c@{\hspace{0.5em}}c@{\hspace{0.5em}}c@{\hspace{0.5em}}c@{\hspace{0.5em}}c}
  %{lccccc}
      \toprule
      Model & Avg. & M.Vista & M.Vision & M.Verse  & WeMath   \\
      \midrule
      % 这里填你的表格内容，示例：
      Self-Sampled& 47.3 & 72.0 & 28.74 & 49.36 & 38.86 \\
      Prior-Filtered & 46.9 & 73.1 & 29.67 & 45.30 & 39.52 \\
      Merge &46.8  & 72.6 & 28.78  & 44.54 & 41.14 \\
      % virl38k  & 73.7 &  & 47.84 &  \\
      \bottomrule
  \end{tabularx}
\end{table}




